Sub-Standards and Mal-Practices: Misinformation's Role in Insular, Polarized, and Toxic Interactions on Reddit

In this work, we examine the influence of unreliable information on political incivility and toxicity on the social media platform Reddit. We show that comments on articles from unreliable news websites are posted more often in right-leaning subreddits and that within individual subreddits, comments, on average, are 32% more likely to be toxic compared to comments on reliable news articles. Using a regression model, we show that these results hold after accounting for partisanship and baseline toxicity rates within individual subreddits. Utilizing a zero-inflated negative binomial regression, we further show that as the toxicity of subreddits increases, users are more likely to comment on posts from known unreliable websites. Finally, modeling user interactions with an exponential random graph model, we show that when reacting to a Reddit submission that links to a website known for spreading unreliable information, users are more likely to be toxic to users of different political beliefs. Our results collectively illustrate that low-quality/unreliable information not only predicts increased toxicity but also polarizing interactions between users of different political orientations.

==> communities.tex <==
\section{Communities}
Having our outlined our techniques for determining the political orientation and toxicity levels of different subreddits, we now turn to understanding how misinformation interacts in subreddits of different political leanings and toxicity levels. 



\subsection{Exponential Random Graph Models}
In order to model some of the interactions between online toxicity, misinformation levels, and polarization levels, we utilize exponential random graphs. Exponential Random Graph Modeling (ERGM), is a network models are a form of random graphs that predict connections between different nodes in a given network~\cite{hunter2008ergm}. ERGM models assume that connections are determined by a random variable $p^*$ that is dependent on input variables.  As in Chen \textit{et al.}~\cite{chen2022misleading} and Peng \textit{et al.}~\cite{peng2016follower}. We utilize this modelling as it does it does not assume that its data input is independent; given that we want to model the interactions of polarization, toxicity, and misinformation levels, this relaxed restriction is key. Furthermore, ERGMs can be efficiently computed with random Markov Chain Monte Carlo processes allowing us to model the large amounts of interactions between subreddits and between user in our dataset~\cite{van2019introduction,hunter2008ergm}.

==> dead.tex <==
\subsection{Twitter Dataset}
 For our Twitter dataset, we collected the Tweets of a set of users that tweeted conspiracy theory, misinformation, or authentic news wesbites from their profile. Utilizing our set of conspiracy theory, misinformation, and authentic news websites and the Python \texttt{Tweepy} we collected the usernames of profiles that tweeted these domains throughout December 2021, totaling 181K different Twitter users. For each of these users, utilizing the \texttt{Tweepy} API we then collected each of their most recent 3240 tweet. Altogether this totaled 446,439,819 different tweets.
 
 In addition, to this core dataset, in order to understand the larger Twitter ecosystem and the relative toxicity and the amounts of misinformation on the platform, we also we utilize the Twitter Streaming API. The Twitter Streaming API gives real-time access to 1\% of public tweets. We continuously collected these tweets between July 10 and and December 21, 2020. We utilize this dataset to understand the characteristics of English language Twitter as a whole. 
 
 
 
 \begin{figure}
    \centering

\begin{tikzpicture}[very thick]
    % Right square
    \node[fill=gray!20,draw=red, minimum size=2cm, inner sep=0pt] (as) {$1.08\%$};
    \node[draw=black,minimum size=2cm, inner sep=0pt, above=-\pgflinewidth of as] (abh) {$0.94\%$};
    \node[draw=black,minimum size=2cm, inner sep=0pt, right=-\pgflinewidth of as] (abv) {$0.87\%$};
    \node[fill=gray!20,draw=blue, minimum size=2cm, inner sep=0pt,  above right=-\pgflinewidth and -\pgflinewidth of as]  {$1.24\%$};
    
    % Side labels
    \node[anchor=east,rotate=90,yshift=0.3cm,xshift=1.0cm] at (as.west) {Conservative};
    \node[anchor=north,] at (as.south) {Liberal};
    \node[anchor=east,rotate=90,yshift=0.3cm,xshift=0.6cm] at (abh.west) {Liberal};
    \node[anchor=north] at (abv.south) {Conservative};
    
    
    % Square label
    \node[xshift=1cm, below=0.7cm of as] {Target};
    
    \node[yshift=1.50cm,xshift=-0.75cm,rotate=90,left=0.5cm of as] {Author};

\end{tikzpicture}
  \caption{Percentage of interactions that are toxic/uncivil in misinformation submissions}
    \label{fig:my_label}
    
\end{figure}    

\begin{figure}
    \centering

\begin{tikzpicture}[very thick]
    % Right square
    \node[fill=gray!20,draw=red, minimum size=2cm, inner sep=0pt] (as) {$0.78\%$};
    \node[draw=black,minimum size=2cm, inner sep=0pt, above=-\pgflinewidth of as] (abh) {$0.83\%$};
    \node[draw=black,minimum size=2cm, inner sep=0pt, right=-\pgflinewidth of as] (abv) {$0.82\%$};
    \node[fill=gray!20,draw=blue, minimum size=2cm, inner sep=0pt,  above right=-\pgflinewidth and -\pgflinewidth of as]  {$0.76\%$};
    
    % Side labels
    \node[anchor=east,rotate=90,yshift=0.3cm,xshift=1.0cm] at (as.west) {Conservative};
    \node[anchor=north,] at (as.south) {Liberal};
    \node[anchor=east,rotate=90,yshift=0.3cm,xshift=0.6cm] at (abh.west) {Liberal};
    \node[anchor=north] at (abv.south) {Conservative};
    
    
    % Square label
    \node[xshift=1cm, below=0.7cm of as] {Target};
    
    \node[yshift=1.50cm,xshift=-0.75cm,rotate=90,left=0.5cm of as] {Author};

\end{tikzpicture}
  \caption{Percentage of interactions that are toxic/uncivil in mainstream submission}
    \label{fig:my_label}
    
\end{figure}   

\begin{table}[b]
\centering
\begin{tabular}{ll}
\toprule
   \multicolumn{2}{c}{\large Toxic Interactions}          \\
   \toprule
      \midrule
      Intercept              & -8.545 ***  &-8.530*** \\               
      \midrule
      User Polarization               & -0.292 & -0.464 \\
      \midrule
      User Polarization Differences    & -2.040*** &-0.782 *** \\
    \midrule
       User Toxicity &   10.557*** &  12.396***\\
      \midrule
       Reciprocity &   3.0863*** &  4.568***\\
      \midrule
\bottomrule
& $\ast p<0.05; ** p<0.01; *** p<0.001$ \\
\end{tabular}
\caption{Caption\label{time}}
\end{table}



\begin{figure}
\begin{minipage}[l]{0.3\textwidth}
\includegraphics[width=1\columnwidth]{figures/subreddit_distribution.png} 
\end{minipage}
\begin{minipage}[l]{0.3\textwidth}
\caption{\textbf{Misinformation, Toxicity, and Political Polarization Interactions}--- As subreddits increase in misinformation levels, they become more toxic. There is not a large correlation between misinformation levels and the political polarization of subreddits.}
\end{minipage}
\label{figure:subreddit_interaction}
\end{figure}


\begin{table}[b]
\centering
\begin{tabular}{lll}
\toprule
   \multicolumn{3}{c}{\large Number of Comments on Misinfo Submissions}          \\
   \toprule
                                  & {Zero Inflated}  & {Negative Binomial }  \\
                      &       \footnotesize{negative coefficient = } &  \footnotesize{positive coefficient = }\\
                      &       \footnotesize{more likely to get comments} &  \footnotesize{more comments}\\
      \midrule
      Intercept              & 5.810*** & 3.290***  \\               
      \midrule
      Absolute User Polarization               & -7.515***  & -3.550***  \\
      \midrule
      Absolute Subreddit Polarization              & 2.700*** &-0.568* \\
    \midrule
       Subreddit Toxicity & -6.395***   & 5.525*** \\
      \midrule
       User Toxicity &   -13.470*** &  -11.750***\\
      \midrule
      Average Subreddit Comments &  -9.112*** & 1.300***  \\
\bottomrule
& $^\ast p<0.05; \;  ^{**} p<0.01; \; ^{***}p<0.001$ \\

\end{tabular}
\end{table}


\begin{table}[b]
\centering
\begin{tabular}{lll}
\toprule
   \multicolumn{3}{c}{\large Number of Comments on Mainstream Submissions}          \\
   \toprule
                            & {Zero Inflated}  & {Negative Binomial }  \\
                      &       \footnotesize{negative coefficient = } &  \footnotesize{positive coefficient = }\\
                      &       \footnotesize{more likely to get comments} &  \footnotesize{more comments}\\
      \midrule
      Intercept              & 3.054***  &2.436*** \\               
      \midrule
     Absolute User Polarization               & -4.463***  & -2.566***  \\
      \midrule
      Absolute Subreddit Polarization              & 4.296*** &0.415 *** \\
    \midrule
      Subreddit Toxicity & 5.298***  & 12.033*** \\
      \midrule
       User Toxicity &   -12.261*** &  -7.558***\\
      \midrule
      Average Subreddit Comments &  -7.712*** & 0.861***  \\
\bottomrule
& $^\ast p<0.05; \;  ^{**} p<0.01; \; ^{***}p<0.001$ \\
\end{tabular}
\end{table}


\begin{table}
    \small
    \centering
    \begin{tabularx}{1\columnwidth}{XrXr}
    \toprule
    {Conservative Subreddits} & Polarization Score & Liberal Subreddits & Polarization Score\\
    \midrule
    {r/The\_Generals\_Corner}  & 0.876 &r/Illinois4Sanders &-0.843\\
    {r/AmericanThinkerForum} & 0.829 &r/Georgia4Sanders &-0.843\\
    {r/PhillyGuns}  &  0.782 &r/NewMexicoForSanders &-0.843\\
    {r/FightingFakeNews} &0.758 &r/alaskaforsanders &-0.843 \\
    {r/HatedForNoReason777} &0.742 &r/dc4sanders &-0.843\\
    \bottomrule
    \end{tabularx}
 \caption{\textbf{The most politically charged subreddits}--- The most liberal subreddits are those advocating for US Senator Bernie Sanders. }
   \label{table:mostpolitical-subreddits}
\end{table}


\begin{table}
    \small
    \centering
    \begin{tabularx}{0.5\columnwidth}{Xr}
    \toprule
    {Most Toxic Subreddits} & Comment Toxic \%\\
    \midrule
    {r/141414} &100\% \\
    {r/ElectionPollsUSA}  &  100\% \\
      {r/spamswearshere}  & 100\% \\
    {r/icummedtothat} &88.4\% \\
    {r/WorshipSofiaVergara} & 81.5\%\\
    
    \bottomrule
    \end{tabularx}
  \caption{\textbf{The Most Toxic Subreddits}}
   %\vspace{-20pt}
   \label{table:website-cllections}
\end{table}

\begin{table}[t]
\centering
\small
\begin{tabular}{ll}
\toprule
 Misinformation Interactions  & Coefficient \\ \midrule
      Intercept               &-8.711*** \\               
     Absolute User Polarization       &         0.882* \\
      User Polarization Differences     & -1.278*** \\
       User Toxicity &  9.003***\\
       User Moderator/Admin Status &   -.04660\\
       Relative User Age (years) &   -0.0049\\
       Reciprocity & 3.569 ***\\
       Shared Subreddits &  0.0004\\
\bottomrule
 $\quad\quad\quad\quad ^\ast p<0.05; \;  ^{**} p<0.01; \; ^{***}p<0.001$ \\
\end{tabular}
\caption{\textbf{Toxic Mainstream Submission Interactions}. As confirmed in our ERGM, differences in political orientation of users is predictive of increased incivility and toxicity. Similarly, the higher each individual user's toxicity norm they are more likely to target other users with toxic comments. }
\label{tbl:ergm}
\end{table}





\begin{table}
    \scriptsize
    \centering
    \begin{tabularx}{0.9\columnwidth}{l|ccc}
    \toprule
   &\multicolumn{1}{c}{{\textbf{\scriptsize{Misinformation Submission}} }} &\multicolumn{1}{c}{{\textbf{\scriptsize{Mainstream Submissions}} }} & \multicolumn{1}{c}{{\textbf{\scriptsize{All Submissions}} }} \\ \midrule
   Toxic Mod/Admin Interactions & 433 (4.15\%)  &  4,991 (2.93\%)& 245,780 (1.8\%)\\
   Mod/Admin Responding Toxicly & 88 (0.84\%) & 945 (0.55\%)& 54,674 (0.40\%)\\
   Mod/Admin Responding to Toxicity & 106 (1.0\%)  &1,365 (0.80\%) &66,477 (0.48\%) \\
    \bottomrule
    \end{tabularx}
  \caption{\textbf{Moderators and admins have similar roles across different submissions.}}
   %\vspace{-20pt}
   \label{table:website-mod-inter}
\end{table}
 \begin{table}[t]
\centering
\small
\begin{tabular}{ll}
\toprule
   \textbf{Misinformation Submissions} \\
      \midrule
      Mod/Admin Toxicity               &$1.38\%\pm0.15\%$ \\          Non-Mod/Admin Toxicity               &$1.25\%\pm0.02\% $\\     \midrule  
      
     \textbf{Authentic News Submissions} \\
      \midrule
      Mod/Admin Toxicity               &$0.91\% \pm0.02\%$\\          Non-Mod/Admin Toxicity.  &$0.64\% \pm0.001\%$\\        \midrule 
      
      \textbf{All Submissions} \\ 
      \midrule
      Mod/Admin Toxicity               &$ 0.46\%\pm0.000\%$\\       
      Non-Mod/Admin Toxicity.  &$1.36\%  \pm0.000\%$\\   
\bottomrule
\end{tabular}
\caption{\% of Toxic Comments w for Moderator/Admin and Non-Moderator/Admin Users on Misinformation, Authentic News, and All Submissions with 95\% Normal Confidence Intervals. }
\label{tbl:ergm}
\end{table}

\begin{table}
    \scriptsize
    \centering
    \begin{tabularx}{0.9\columnwidth}{l|ccc}
    \toprule
   &\multicolumn{1}{c}{{\textbf{\scriptsize{Misinformation Submission}} }} &\multicolumn{1}{c}{{\textbf{\scriptsize{Mainstream Submissions}} }} & \multicolumn{1}{c}{{\textbf{\scriptsize{All Submissions}} }} \\ \midrule
   Toxic Mod/Admin Interactions &  4.15\%  &  2.93\%& 1.8\%\\
   Mod/Admin Responding Toxicly & 0.84\% & 0.55\% &0.40\% \\
   Mod/Admin Responding to Toxicity & 1.00\%  &0.80\% &0.48\% \\
    \bottomrule
    \end{tabularx}
  \caption{{Moderators and admins have similar roles across different submissions.} Across all types of interactions, moderators tend to respond more to toxic comments than post toxic comments themselves. }
   \vspace{-15pt}
   \label{table:website-mod-inter}
\end{table}

\begin{figure}
\begin{subfigure}{.48\textwidth}
  \centering
 \includegraphics[width=1\columnwidth]{figures/subreddit_correlation_toxicity-20240428.pdf} 
\end{subfigure}
\begin{subfigure}{.48\textwidth}
  \centering
 \includegraphics[width=1\columnwidth]{figures/user_correlation_toxicity-20240428.pdf} 
\end{subfigure}
 \caption{Correlations between the politicalness, toxicity, and partisanship of subreddits an users.\label{figure:all_correlations}}
 \vspace{-10pt}
\end{figure}

==> interactions.tex <==
\section{Reddit Level Interactions}
As found in prior work, subreddits maintain particular levels of toxicity community norms~\cite{rajadesingan2020quick}. For example, as found by Rajadesingan \textit{et al.}, the subreddit WhiteRights had much higher tolerance for toxic content than the subreddits NeutralPolitics or AskEconomics. In this section, we analyze how distinctive political norms and toxicity levels within given subreddits contribute to levels of misinformation. 


In order to get an approximation of the levels of misinformation within a given subreddit we utilize a set of 157,605 \textit{misinformation-oriented} websites. We define \textit{misinformation-oriented} websites as websites that have more connections from our set of misinformation websites than from authentic news (i.e., the majority of a site's inward links in a domain-based graph are from misinformation websites. Websites that have been widely documented as spreading falsehood and conspiracy theories are included within this list including InfoWars and 8kun.top~\cite{hanley2022no,starbird2018ecosystem}.


As seen in Figure~\ref{figure:misinfo-toxciity-polarization}, there are political and toxicity norms across the spectrum, with polarization levels not being correlated levels of toxicity nor with misinformation levels. We see in particular that subreddits that are at the edge of political spectrum actually have some of the lowest average Perspective Toxicity scores and the lowest amounts of misinformation hyperlinks. We thus see at that at the edges of the political spectrum, where users are more isolated and insular that the overall levels of toxicity within the subreddit are not as high as those more ``moderate'' subreddits. This suggests that these cohesive communities where users are more similar to each other may producing the least amounts of bad behavioral outcomes. 


As seen in Figure~{}, toxicity the


\begin{figure}
\centering
\includegraphics[width=0.75\columnwidth]{figures/subreddit_distribution.png} 
\caption{\textbf{Distributions of political polarization, perspective toxicity levels, and misinformation-oriented URL usage across subreddits with at least 100 users }--- While previous research has indicated that political polarization and toxicity are heavily correlated, we see in Reddit's case due to its self-selecting communities that political polarization is not correlated with vitriol and comment toxicity. Similarly we see that political polarization is not correlated with misinformation levels. Rather subreddits within the political center have the highest percentages of misinformation and toxicity. 
}
\label{figure:misinfo-toxciity-polarization}
\end{figure}

==> reddit.tex <==
\section{Moderating Influences: Community Based Control on Misinformation Spread}
In this section, we examine the different misinformation ecosystems on Reddit. Largely in contrast to the self-organizing and porous communities that exist on Twitter, Reddit allows users to  establish their own self-contained communities. These communities known as subReddits have their own rules, communities norms, political preferences, as well as purposes. These subReddits module, control, and filter the content on Reddit platform. Behaviors in one subReddit that blocked or condemned in one subReddit can be widely celebrated in another subReddit. For example, one subReddit \texttt{r/conspiracy} that has over 1.7M (at time of writing in February 2022)  is dedicated to the discussion on conspiracy theories. Conspiracy Theories that are widely discussed in this subReddit are often ridiculed in other subReddit like \texttt{r/Qult\_Headquarters}.
\begin{figure*}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/average-toxicity-end-2020.png}
\label{fig:cdf-subreddit-hyperlinks}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/average-toxicity-distribution-end2020.png}
 \label{fig:cdf-user-hyperlinks}
\end{subfigure}
\label{fig:cdf-hyperlinsk}
\caption{\textbf{Relative Perspective API toxicity of tweets and comments on Twitter and Reddit}--- Comparing a 1\% Twitter stream's Perspective API toxicity scores to the bulk of Reddit comments from  July to December 2020, we see that Reddit has maintained lower levels of toxicity over time and amongst users. }
\end{figure*}


\begin{figure*}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/polarization_redidit_twitter.png}
\label{fig:cdf-subreddit-hyperlinks}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/average-toxicity-distribution-end2020.png}
 \label{fig:cdf-user-hyperlinks}
\end{subfigure}
\label{fig:cdf-hyperlinsk}
\caption{\textbf{Relative Perspective toxicity of tweets and comments on Twitter and Reddit}--- Comparing a 1\% Twitter stream's Perspective API toxicity scores to the bulk of Reddit comments from  July to Decemebr 2020, we see that Reddit has maintained lower levels of toxicity over time and amongst users. }
\end{figure*}
As seen in Figures~\ref{}

Because of self-organizing and fairly norm-heavy communities form on Reddit, we find that our set of misinformation URLs are largely confined to a small set of subReddits and set of users. As seen in Figure~\ref{fig:cdf-subreddit-hyperlinks}, fairly few subReddits are responsible for the amount of Misinformation URLs Reddit Submissions. For instance, we find that only 133 Reddits were responsible for 90\% of Misinformation URL submission on Reddit from July 2020 to December 2020. Only 4007 contained misinformation URLS within their submissions. 4878 different subReddits contained misinformation URLs in their comments.While some of misinformation posts could have been removed by moderators and Reddit itself, this illustrates the moderating effect community norms have on the material that is posted and stays posted in  the majority of subreddits. This is largely in contrast to the number of subReddits containing authentic news URLs, with 513 subReddits containing 90\% of authentic news URL submissions and 12,825 containing authentic news Reddit Submissions. 18131 different subReddits had authentic news domain hyperlinks in their comments from July 2020 to December 2020. This behavior among subreddits largely caries over to the set of Reddit users who posted these links to misinformation and authentic news websites. As seen in Figure~\ref{fig:cdf-user-hyperlinks}, just 1423 users were responsible for 90.0\% of of misinformation URLs subReddit submissions in contrast to the 11,336 responsible for authentic news submissions. 
\begin{figure*}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/misinformation-authentic-cdf.png}
  \caption{\textbf{CDF News Hyperlinks by Subreddit}— Just 133 subreddits posted  90.0\% of hyperlinks to the misinformation websites in our dataset from July 2020 to December 2020. In contrast, 513 subReddits posted 90.0\% of the hyperlinks to authentic news websites during this same period. 
}
\label{fig:cdf-subreddit-hyperlinks}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/misinformation-authentic-users-cdf.png}
 \caption{\textbf{CDF News Hyperlinks by User}— Just 1423 subreddits posted  90.0\% of hyperlinks to the misinformation websites in our dataset from July 2020 to December 2020. In contrast, a whopping 11,336 subReddits posted 90.0\% of the hyperlinks to authentic news websites during this same period. 
}
 \label{fig:cdf-user-hyperlinks}
\end{subfigure}
\label{fig:cdf-hyperlinsk}
\end{figure*}


\begin{figure*}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/partisanship_avg.png}
 
\label{fig:partisanship-average}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/toxicity_avg.png}
 
 \label{fig:toxicity-average}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/partisanship_variance.png}
 
\label{fig:partisanship-variance}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/toxicity_variance.png}
 
 \label{fig:toxicity-variance}
\end{subfigure}
\caption{\textbf{Toxicity and Political URL Variation among Users and SubReddits }--- As seen above, there are relatively tight windows of political partisanship and toxicity among subreddits with subreddits having approximately little more diversity than individual users. 
}
\label{fig:diversity-of-views}
\end{figure*}
\begin{figure*}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/numberOfSubRedditsByPartianshipAvg.png}
  \caption{\textbf{User SubReddit Paritipation vs Variance in Political URLs Posted}-
}
\label{fig:participation-political}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/numberOfSubRedditsByToxicityAvg.png}
 \caption{\textbf{User SubReddit Paritipation vs Variance in Comment Toxicity}— 
}
 \label{fig:participation-toxicity}
\end{subfigure}
\caption{\textbf{Relative amounts of partisanship and toxicity diversity among individual users by SubReddit participation }--- As users participate in more and more the variance of their behavior increases with user posting a wider variety of political websites and commenting with a wider berth of toxicity. 
}
\label{fig:participation}
\end{figure*}
The moderating effect of subReddits is further seen in the relatively narrow window of political views and level of toxicity that are allowed within each subReddit community. As seen in Figure~\ref{fig:diversity-of-views}, there relatively narrow windows of allowed divergence in political beliefs and toxicity among SubRedits and users. This is in Figure~\ref{fig:participation}, as only as users participate in more and more subReddits does the berth of different types of comments that they post increase. On average, after a user participates in TODO subreddits the variance of their toxicity exceeds the average subReddit (an entire community). This illustrates the ability of subReddit communities to maintain an equilibrium of acceptable toxicity on their platforms, excising redditors who go outside normal bounds as illutrated in prior work~\cite{rajadesingan2020quick}.  Similarly, we find  that as users participate and post in more subReddits, they post a wider political range of websites.


\begin{figure*}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/user-partisanship-var.png}
  \caption{\textbf{Number of SubReddit Users vs Variance in Political URLs Posted}-
}
\label{fig:participation-political}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/user-toxicity-var.png}
 \caption{\textbf{Number of SubReddit Users vs Variance in Comment Toxicity}— 
}
 \label{fig:participation-toxicity}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/partisanship-to-num-subreddits.png}
 
\label{fig:particiption-median-toxicity}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/toxicity-to-num-subreddits.png}

 \label{fig:cdf-user-hyperlinks}
\end{subfigure}
\label{fig:cdf-hyperlinsk}
\caption{\textbf{Number of Users to Variance in SubReddit Behavior}--- As the number of users in a particular subReddit increases, there is no discernible trend in the the variance of political URLS posted nor the Perspective API toxicity. However, as the the number of subReddits that the median user participates in increases within a given subReddit, the variance in political URLs and the the variance in toxicity does increase.  
}
\label{fig:participation}
\end{figure*}

Conversely, we find that the number of users that a subReddit contains, does not correlate with the diversity of toxicity and political views present on that subReddit. As seen in Figure~\ref{fig:participation}, as the number of users that post submissions in a subReddit increases, there is no discernible correlation with the variance of toxicity nor the variance of political views voiced on that subReddit. In contrast, we find that as the median subReddit participation on Reddit increases, the variance of toxicity and political viewd does increase.  Namely, if a subReddit has users that participate in a wide range of subReddits outside that particular subReddit, then this particular subReddit has higher levels of variance in political views and toxicity. This suggests that amount of people that a subReddit does not correspond with diversity of views and behavior on that subReddit but rather with the amount of communities that that subReddit's users come from and with which they engages. 
\begin{figure*}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/user-misinfo-toxicity.png}
\label{fig:user-misnformation}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/reddit-misinfo-toxicity.png}
 \label{fig:reddit-misinformation}
\end{subfigure}
\label{fig:misinformation-reddit-user}
\end{figure*}
Having established how the characteristics of subReddits exerts norms over their particular users, we now turn to understand how these norms affect the levels of misinformation on Reddit platform and on particular subReddits. 
As seen in Figure~\ref{fig:misinformation-reddit-user}, as on Twitter, misinformation subReddits as well as have higher levels of toxicity compared with subReddis with not misinformatino submissions. 

Looking a







==> twitter.tex <==
\section{Borderless: Twitter Misinformation and Political Communities}
In this section, we analyze the interplay between the penchant towards political polarization, toxicity, and misinformation on social media users. Previous works have indicated that toxicity levels are heavily tied with users' political polarization levels~\cite{chipidza2021effect,kim2021distorting} as well as their penchant to conspiratorial content~\cite{hanley2021no}. We now investigate how toxic and political polarized communities contribute to the propagation of misinformation and conspiracies by individuals users on Twitter.  

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/LevelsOfMisinformationAndNewsOnTwitter.png} 
\caption{\textbf{Number of Authentic News, Misinformation, and Conspiracy Theory Links on Twitter in 2020}--- Misinformation maintains a large presence of Twitter, with about half as many links as authentic news. Conspiracy websites having a relatively small but non-negligible presence on the platform. 
}
\label{figure:levels_of_misinfo}
\end{figure}

As seen in Figure~\ref{figure:levels_of_misinfo}, counting the number of instances of misinformation, authentic news, and conspiracy theory hyperlinks based on a 1\% Twitter sampling over 6 months, there are consistent levels of misinformation news articles tweeted. The amount of misinformation links from users, in fact largely follows the amount of authentic news tweeted. Specifically, we find a Pearson correlation of 0.711 between the number of misinformation URLs posted and the number of authentic news posted.  At any given time, the amount of misinformation links within our dataset varies from, $\frac{1}{3}$ to $\frac{1}{2}$ of the amount of authentic news hyperlinks posted. Comparing this to a set of non-news related URLS as well as a set of random domains (chosen randomly from the Amazon Alexa Top 1M from January 1 2022), we see that the changing amounts of misinformation and news based URLs in our dataset is largely due to the vicissitudes of the news cycles rather than as an artifact of our dataset. 

Having established the relative levels of misinformation on Twitter, we now seek to understand some of the drivers behind misinformation heavy Twitter accounts. Taking all URLS within our dataset, we acquire 189K different Twitter accounts that tweets authentic news, misinformation, or conspiracy theories during the month of January. Within this set of Twitter accounts 139663 accounts tweeted at least one authentic news website and 115073 accounts tweeted at least one misinformation website. Using the Tweepy API, we collect the last 3240 tweets of each of these users, giving us a dataset of 446,439,819 tweets total. 

\begin{figure*}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/all-correlations.png}
  \caption{All User Correlations}
\label{fig:twitter-reddit-partisanship-time}
\end{subfigure}%
\hspace{20pt}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/republican-correlations.png}
  \caption{Republican User Correlations}
  \label{fig:twitter-reddit-partisanship}
\end{subfigure}
\hspace{20pt}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/democratic-correlations.png}
  \caption{Democratic User Correlations}
  \label{fig:twitter-reddit-toxicity-time}
\end{subfigure}
\caption{\textbf{Twitter User Characteristic Correlations}--- Among different 
}
\label{fig:twitter-correlations}
\end{figure*}

After labeling each tweet with the Perspective API and gathering each accounts approximate partisanship, partisanship URL variance, and misinformation promotion levels, we now seek to understand the factors behind accounts promoting misinformation. As a proxy for the misinformation promotion level of given Twitter users, we utilize the percentage of the URLs that they post that belong to our set of misinformation domains.

As seen in Figure~\ref{fig:twitter-correlations}, there is a high degree of correlation between the political polarization of users and misinformation levels of users. This largely concurs with prior research that suggests that political polarization is the most potent reason behind the sharing of ``fake-news'' on Twitter~\cite{osmundsen2021partisan}. Looking at users whose average URL posted is conservative/Republican, this is especially prominent,  with polarization having a 0.70 Pearson correlation with levels of misinformation on their accounts. 


We also see, somewhat counter-intuitively, at a given level of partisanship, as the partisanship variance of individuals accounts increases, the amount of misinformation that that account post also increases. This suggests that users that actually engage with materials/hyperlink to materials that are substantially different from the average political information that they hyperlink to are more likely to post misinformation. Bucking our initial expectations, engaging with more and different sources is associated with heavier amounts of misinformation. Prior work~\cite{starbird2018ecosystem} has noted the political echo chambers that promote misinformation online. However, this appears to be only a part of the story of the spread of misinformation. 
\begin{comment}
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/misinformation-graph-partisan-var.png} 
\caption{\textbf{Partisanship and Partisanship Variance Affect on Misinformation}--- As users become more politically hardened and engage with a higher amount of news sources, they are more likely to post misinformation. While not exact, as levels of variety of political URLS posted increases at each level of partisanship, the the levels of misinformation increases as well. This is seen by the red fraying at the edges of the graph.  
}
\label{figure:partisanship-misinfo-variance}
\end{figure}
\end{comment}
As seen in Figure~\ref{figure:partisanship-misinfo-variance}, it is the set of users that have the highest variance of political URLs as well as the most highly partisan users that have the highest levels of misinformation on their Twitter accounts.For example one particularly highly misinformation-dense account (Figure~\ref{fig:twitter-misinformation2}) linked to a video from MSNBC to deride one of its hosts. This is not to say that these users regularly link to highly opposing views often; however, this tendency to interact with substantially different than a user's political average results in a higher likelihood of misinformation. 
\begin{figure*}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/liberal-graph-partisan-misinformation.png}
\label{fig:left-twitter-pol-toxicity}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/conservative-graph-partisan-misinformation.png}
  \label{fig:right-twitter-pol-toxicity}
\end{subfigure}
\caption{\textbf{Average Misinformation Levels as a function of average political bias and tendency to post opposing views}-- Users that post the URLs of websites that are against their average political bias are more likely to post misinformation.
}
\label{fig:twitter-pol-toxicity}
\end{figure*}

Users that post more URLs that are opposed to their mean political URLs/belief also show a higher probability of toxicity compared to other users of similar political averages. Plotting levels of toxicity as a function of political bias and the tendency to post opposing views (URLs from websites that are conservative-leaning for Democratic voters and vice versa), we see 1) that levels of toxicity are highly connected with levels of partisanship ( Pearson correlation of 0.38 for all users), and 2) that as the number of URLs from websites with opposing views increases, we see that average levels of toxicity increase as well. Looking at Figure \ref{fig:twitter-pol-toxicity} and , we  that for both left-wing and right-wing users, similarity at each given partisanship level, as the percentage of URLs from websites that oppose their mean political bias increases, that mean levels of toxicity increases with users at the end of each level of partisanship showing the highest levels of toxicity. For liberal leaning users, we find that after normalizing for partisanship, a Pearson correlation of 0.242 between the average toxicity of a user and their tendency to post URLs opposing their political bias. Just looking at decidedly conservative users with an average political bias of 0.1 or greater, this correlation increases to 0.302. For conservative users, we find that after normalizing for partisanship, the tendency to post opposing views accounts, has a Pearson correlation of 0.240 with their average toxicity. Just looking at decidedly conservative users with an average political bias of 0.1 or greater, this correlation increases to 0.302. As seen, users with the tendency to post URLS against their political bias have higher associated levels of toxicity. This largely mirrors  the tendency to also post misinformation as previously discussed. 

\begin{figure*}
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/high-var-user-tweet1.png}
\label{fig:twitter-misinformation1}
\end{subfigure}%
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/high-var-user-tweet2.png}
  \label{fig:twitter-misinformation2}
\end{subfigure}
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/high-var-user-tweet3.png}
  \label{fig:twitter-misinformation3}
\end{subfigure}
\caption{\textbf{Examples of partisan users engaging with material from across the political aisle }-- Highly partisan and misinformation dense Twitter accounts occasional respond to and engage with news stories from authentic news. As pictured, users often deride these sources or cite that stories are  highly divisive.
}
\label{fig:twitter-misinformation-levels}
\end{figure*}

%% Likelihood to post a right-leaning URL if left wing vs probability to post a left-wing URL if right leaning as a function of partisanship 
\begin{figure*}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/republican-democratic-graph.png}
  \caption{Partisanship Levels}
\label{fig:twitter-average-partisanship}
\end{subfigure}%
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/partisan-variance-graph.png}
  \caption{Partisanship Variance}
  \label{fig:twitter-variance-partisanship}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/toxicity-graph.png}
  \caption{Perspective Toxicity }
  \label{fig:twitter-toxicity}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/misinformation-graph.png}
  \caption{Misinformation }
  \label{fig:twitter-misinformation}
\end{subfigure}
\vspace{5pt}
\caption{\textbf{Interconnections between Twitter users with corresponding levels of partisanship, levels of sharing differently partisan sourced articles, toxicity, and levels of misinformation }-- As seen in the above graphs, highly conservative/Republican users and highly democratic/Republican users largely reference each other. Among these highly polarized communities, these users share more disparate and polarized articles, spread more misinformation, and are more toxic.
}
\label{fig:graph-correlations}
\end{figure*}

The tendency of user with higher levels of toxicity, higher levels of partisanship, and higher likelihoods to post misinformation further carries over to Twitter communities that many of these users participate in. Looking at the set of Twitter users in our scrape that posted at leas 300 URL (top 30K users in our dataset), we see this distinction visually. We plot Twitter mention graphs with edge weights based on how often each user mentions other users in their Tweets. Based on how often each user mentions another and clustering the graph using the Force Atlas 2 algorithm, we see two distinctive clusters of conservative/Republican and liberal/Democratic users form. As seen in Figure~\ref{fig:twitter-average-partisanship}, highly partisan users largely group and interact together, with conservative users mentioning other conservative users more frequently and vice versa. Looking a homophily (the tendency of users to mention/reference users of similar political bias as themselves) we see a moderately high value of 0.604. Comparing the graphs, in


As seen in Figure~\ref{fig:graph-correlations}, the cluster of highly liberal/Democratic and highly conservative/Republican users (Figure ~\ref{fig:twitter-average-partisanship}) corresponds to the set of users with higher amounts of political variance in the URLs that they tweet (Figure ~\ref{fig:twitter-variance-partisanship}) as well as the higher amounts of misinformation (Figure ~\ref{fig:twitter-misinformation}).

Looking at the graph of partisanship variance and the the graph of partisanship levels in Figure~\ref{fig:graph-correlations}, and the corresponding levels of correlation in between partisanship and partisanship variance, the most highly partisan accounts are the ones that hyperlink to a variety of different sources. This is particular true of Republican/conservative users. This can be most clearly seen in the dark pink cluster of the partisanship variance graph corresponding heavily with the Conservative/Republican red of the partisanship levels cluster, and finally dark orange cluster of the misinformation graph. 

